Decoupling the rotation of stars and gas -- I: the relationship with morphology and halo spin

We use a combination of data from the MaNGA survey and MaNGA-like observations in IllustrisTNG100 to determine the prevalence of misalignment between the rotational axes of stars and gas. This census paper outlines the typical characteristics of misaligned galaxies in both observations and simulations to determine their fundamental relationship with morphology and angular momentum. We present a sample of ~4500 galaxies from MaNGA with kinematic classifications which we use to demonstrate that the prevalence of misalignment is strongly dependent on morphology. The misaligned fraction sharply increases going to earlier morphologies (28$\pm$3% of 301 early-type galaxies, 10$\pm$1% of 677 lenticulars and 5.4$\pm$0.6% of 1634 pure late-type galaxies). For early-types, aligned galaxies are less massive than the misaligned sample whereas this trend reverses for lenticulars and pure late-types. We also find that decoupling depends on group membership for early-types with centrals more likely to be decoupled than satellites. We demonstrate that misaligned galaxies have similar stellar angular momentum to galaxies without gas rotation, much lower than aligned galaxies. Misaligned galaxies also have a lower gas mass than the aligned, indicative that gas loss is a crucial step in decoupling star-gas rotation. Through comparison to a mock MaNGA sample, we find that the strong trends with morphology and angular momentum hold true in IllustrisTNG100. We demonstrate that the lowered angular momentum is, however, not a transient property and that the likelihood of star-gas misalignment at z = 0 is correlated with the spin of the dark matter halo going back to z = 1.

==> biblio.tex <==
@ARTICLE{nair2010,
       author = {{Nair}, Preethi B. and {Abraham}, Roberto G.},
        title = "{A Catalog of Detailed Visual Morphological Classifications for 14,034 Galaxies in the Sloan Digital Sky Survey}",
      journal = {\apjs},
     keywords = {catalogs, galaxies: fundamental parameters, galaxies: photometry, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Feb",
       volume = {186},
       number = {2},
        pages = {427-456},
          doi = {10.1088/0067-0049/186/2/427},
archivePrefix = {arXiv},
       eprint = {1001.2401},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJS..186..427N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{westfall2019,
       author = {{Westfall}, Kyle B. and {Cappellari}, Michele and
         {Bershady}, Matthew A. and {Bundy}, Kevin and {Belfiore}, Francesco and
         {Ji}, Xihan and {Law}, David R. and {Schaefer}, Adam and
         {Shetty}, Shravan and {Tremonti}, Christy A. and {Yan}, Renbin and
         {Andrews}, Brett H. and {Brownstein}, Joel R. and {Cherinka}, Brian and
         {Coccato}, Lodovico and {Drory}, Niv and {Maraston}, Claudia and
         {Parikh}, Taniya and {S{\'a}nchez-Gallego}, Jos{\'e} R. and
         {Thomas}, Daniel and {Weijmans}, Anne-Marie and
         {Barrera-Ballesteros}, Jorge and {Du}, Cheng and {Goddard}, Daniel and
         {Li}, Niu and {Masters}, Karen and {Ibarra Medel}, H{\'e}ctor Javier and
         {S{\'a}nchez}, Sebasti{\'a}n F. and {Yang}, Meng and {Zheng}, Zheng and
         {Zhou}, Shuang},
        title = "{The Data Analysis Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey: Overview}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jan",
          eid = {arXiv:1901.00856},
        pages = {arXiv:1901.00856},
archivePrefix = {arXiv},
       eprint = {1901.00856},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190100856W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{belfoire2019,
       author = {{Belfiore}, Francesco and {Westfall}, Kyle B. and {Schaefer}, Adam and
         {Cappellari}, Michele and {Ji}, Xihan and {Bershady}, Matthew A. and
         {Tremonti}, Christy and {Law}, David R. and {Yan}, Renbin and
         {Bundy}, Kevin and {Shetty}, Shravan and {Drory}, Niv and
         {Thomas}, Daniel and {Emsellem}, Eric and
         {S{\'a}nchez}, Sebasti{\'a}n F.},
        title = "{The Data Analysis Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey: Emission-Line Modeling}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jan",
          eid = {arXiv:1901.00866},
        pages = {arXiv:1901.00866},
archivePrefix = {arXiv},
       eprint = {1901.00866},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190100866B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gunn2006,
   author = {{Gunn}, J.~E. and {Siegmund}, W.~A. and {Mannery}, E.~J. and 
	{Owen}, R.~E. and {Hull}, C.~L. and {Leger}, R.~F. and {Carey}, L.~N. and 
	{Knapp}, G.~R. and {York}, D.~G. and {Boroski}, W.~N. and {Kent}, S.~M. and 
	{Lupton}, R.~H. and {Rockosi}, C.~M. and {Evans}, M.~L. and 
	{Waddell}, P. and {Anderson}, J.~E. and {Annis}, J. and {Barentine}, J.~C. and 
	{Bartoszek}, L.~M. and {Bastian}, S. and {Bracker}, S.~B. and 
	{Brewington}, H.~J. and {Briegel}, C.~I. and {Brinkmann}, J. and 
	{Brown}, Y.~J. and {Carr}, M.~A. and {Czarapata}, P.~C. and 
	{Drennan}, C.~C. and {Dombeck}, T. and {Federwitz}, G.~R. and 
	{Gillespie}, B.~A. and {Gonzales}, C. and {Hansen}, S.~U. and 
	{Harvanek}, M. and {Hayes}, J. and {Jordan}, W. and {Kinney}, E. and 
	{Klaene}, M. and {Kleinman}, S.~J. and {Kron}, R.~G. and {Kresinski}, J. and 
	{Lee}, G. and {Limmongkol}, S. and {Lindenmeyer}, C.~W. and 
	{Long}, D.~C. and {Loomis}, C.~L. and {McGehee}, P.~M. and {Mantsch}, P.~M. and 
	{Neilsen}, Jr., E.~H. and {Neswold}, R.~M. and {Newman}, P.~R. and 
	{Nitta}, A. and {Peoples}, Jr., J. and {Pier}, J.~R. and {Prieto}, P.~S. and 
	{Prosapio}, A. and {Rivetta}, C. and {Schneider}, D.~P. and 
	{Snedden}, S. and {Wang}, S.-i.},
    title = "{The 2.5 m Telescope of the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0602326},
 keywords = {Surveys, Telescopes},
     year = 2006,
    month = apr,
   volume = 131,
    pages = {2332-2359},
      doi = {10.1086/500975},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.2332G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smee2013,
   author = {{Smee}, S.~A. and {Gunn}, J.~E. and {Uomoto}, A. and {Roe}, N. and 
	{Schlegel}, D. and {Rockosi}, C.~M. and {Carr}, M.~A. and {Leger}, F. and 
	{Dawson}, K.~S. and {Olmstead}, M.~D. and {Brinkmann}, J. and 
	{Owen}, R. and {Barkhouser}, R.~H. and {Honscheid}, K. and {Harding}, P. and 
	{Long}, D. and {Lupton}, R.~H. and {Loomis}, C. and {Anderson}, L. and 
	{Annis}, J. and {Bernardi}, M. and {Bhardwaj}, V. and {Bizyaev}, D. and 
	{Bolton}, A.~S. and {Brewington}, H. and {Briggs}, J.~W. and 
	{Burles}, S. and {Burns}, J.~G. and {Castander}, F.~J. and {Connolly}, A. and 
	{Davenport}, J.~R.~A. and {Ebelke}, G. and {Epps}, H. and {Feldman}, P.~D. and 
	{Friedman}, S.~D. and {Frieman}, J. and {Heckman}, T. and {Hull}, C.~L. and 
	{Knapp}, G.~R. and {Lawrence}, D.~M. and {Loveday}, J. and {Mannery}, E.~J. and 
	{Malanushenko}, E. and {Malanushenko}, V. and {Merrelli}, A.~J. and 
	{Muna}, D. and {Newman}, P.~R. and {Nichol}, R.~C. and {Oravetz}, D. and 
	{Pan}, K. and {Pope}, A.~C. and {Ricketts}, P.~G. and {Shelden}, A. and 
	{Sandford}, D. and {Siegmund}, W. and {Simmons}, A. and {Smith}, D.~S. and 
	{Snedden}, S. and {Schneider}, D.~P. and {SubbaRao}, M. and 
	{Tremonti}, C. and {Waddell}, P. and {York}, D.~G.},
    title = "{The Multi-object, Fiber-fed Spectrographs for the Sloan Digital Sky Survey and the Baryon Oscillation Spectroscopic Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1208.2233},
 primaryClass = "astro-ph.IM",
 keywords = {cosmology: observations, instrumentation: spectrographs, surveys },
     year = 2013,
    month = aug,
   volume = 146,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-6256/146/2/32},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....146...32S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{drory2015,
   author = {{Drory}, N. and {MacDonald}, N. and {Bershady}, M.~A. and {Bundy}, K. and 
	{Gunn}, J. and {Law}, D.~R. and {Smith}, M. and {Stoll}, R. and 
	{Tremonti}, C.~A. and {Wake}, D.~A. and {Yan}, R. and {Weijmans}, A.~M. and 
	{Byler}, N. and {Cherinka}, B. and {Cope}, F. and {Eigenbrot}, A. and 
	{Harding}, P. and {Holder}, D. and {Huehnerhoff}, J. and {Jaehnig}, K. and 
	{Jansen}, T.~C. and {Klaene}, M. and {Paat}, A.~M. and {Percival}, J. and 
	{Sayres}, C.},
    title = "{The MaNGA Integral Field Unit Fiber Feed System for the Sloan 2.5 m Telescope}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1412.1535},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: general, instrumentation: spectrographs, surveys, techniques: imaging spectroscopy},
     year = 2015,
    month = feb,
   volume = 149,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-6256/149/2/77},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....149...77D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{law2015obs,
   author = {{Law}, D.~R. and {Yan}, R. and {Bershady}, M.~A. and {Bundy}, K. and 
	{Cherinka}, B. and {Drory}, N. and {MacDonald}, N. and {S{\'a}nchez-Gallego}, J.~R. and 
	{Wake}, D.~A. and {Weijmans}, A.-M. and {Blanton}, M.~R. and 
	{Klaene}, M.~A. and {Moran}, S.~M. and {Sanchez}, S.~F. and 
	{Zhang}, K.},
    title = "{Observing Strategy for the SDSS-IV/MaNGA IFU Galaxy Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1505.04285},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, methods: observational, surveys, techniques: imaging spectroscopy},
     year = 2015,
    month = jul,
   volume = 150,
      eid = {19},
    pages = {19},
      doi = {10.1088/0004-6256/150/1/19},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....150...19L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yan2016obs,
   author = {{Yan}, R. and {Bundy}, K. and {Law}, D.~R. and {Bershady}, M.~A. and 
	{Andrews}, B. and {Cherinka}, B. and {Diamond-Stanic}, A.~M. and 
	{Drory}, N. and {MacDonald}, N. and {S{\'a}nchez-Gallego}, J.~R. and 
	{Thomas}, D. and {Wake}, D.~A. and {Weijmans}, A.-M. and {Westfall}, K.~B. and 
	{Zhang}, K. and {Arag{\'o}n-Salamanca}, A. and {Belfiore}, F. and 
	{Bizyaev}, D. and {Blanc}, G.~A. and {Blanton}, M.~R. and {Brownstein}, J. and 
	{Cappellari}, M. and {D'Souza}, R. and {Emsellem}, E. and {Fu}, H. and 
	{Gaulme}, P. and {Graham}, M.~T. and {Goddard}, D. and {Gunn}, J.~E. and 
	{Harding}, P. and {Jones}, A. and {Kinemuchi}, K. and {Li}, C. and 
	{Li}, H. and {Maiolino}, R. and {Mao}, S. and {Maraston}, C. and 
	{Masters}, K. and {Merrifield}, M.~R. and {Oravetz}, D. and 
	{Pan}, K. and {Parejko}, J.~K. and {Sanchez}, S.~F. and {Schlegel}, D. and 
	{Simmons}, A. and {Thanjavur}, K. and {Tinker}, J. and {Tremonti}, C. and 
	{van den Bosch}, R. and {Zheng}, Z.},
    title = "{SDSS-IV MaNGA IFS Galaxy Survey{\mdash}Survey Design, Execution, and Initial Data Quality}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1607.08613},
 keywords = {galaxies: evolution, galaxies: general, surveys, techniques: imaging spectroscopy},
     year = 2016,
    month = dec,
   volume = 152,
      eid = {197},
    pages = {197},
      doi = {10.3847/0004-6256/152/6/197},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152..197Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{law2016drp,
   author = {{Law}, D.~R. and {Cherinka}, B. and {Yan}, R. and {Andrews}, B.~H. and 
	{Bershady}, M.~A. and {Bizyaev}, D. and {Blanc}, G.~A. and {Blanton}, M.~R. and 
	{Bolton}, A.~S. and {Brownstein}, J.~R. and {Bundy}, K. and 
	{Chen}, Y. and {Drory}, N. and {D'Souza}, R. and {Fu}, H. and 
	{Jones}, A. and {Kauffmann}, G. and {MacDonald}, N. and {Masters}, K.~L. and 
	{Newman}, J.~A. and {Parejko}, J.~K. and {S{\'a}nchez-Gallego}, J.~R. and 
	{S{\'a}nchez}, S.~F. and {Schlegel}, D.~J. and {Thomas}, D. and 
	{Wake}, D.~A. and {Weijmans}, A.-M. and {Westfall}, K.~B. and 
	{Zhang}, K.},
    title = "{The Data Reduction Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1607.08619},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, surveys, techniques: imaging spectroscopy},
     year = 2016,
    month = oct,
   volume = 152,
      eid = {83},
    pages = {83},
      doi = {10.3847/0004-6256/152/4/83},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152...83L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cappellari2004,
   author = {{Cappellari}, M. and {Emsellem}, E.},
    title = "{Parametric Recovery of Line-of-Sight Velocity Distributions from Absorption-Line Spectra of Galaxies via Penalized Likelihood}",
  journal = {\pasp},
   eprint = {astro-ph/0312201},
 keywords = {Galaxies: Individual: NGC Number: NGC 3384, Galaxies: Kinematics and Dynamics, line: profiles, Methods: Numerical},
     year = 2004,
    month = feb,
   volume = 116,
    pages = {138-147},
      doi = {10.1086/381875},
   adsurl = {http://adsabs.harvard.edu/abs/2004PASP..116..138C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{cappellari2017,
   author = {{Cappellari}, M.},
    title = "{Improving the full spectrum fitting method: accurate convolution with Gauss-Hermite functions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.08538},
 keywords = {techniques: radial velocities, techniques: spectroscopic, galaxies: kinematics and dynamics},
     year = 2017,
    month = apr,
   volume = 466,
    pages = {798-811},
      doi = {10.1093/mnras/stw3020},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466..798C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{sanchez2006,
   author = {{S{\'a}nchez-Bl{\'a}zquez}, P. and {Peletier}, R.~F. and {Jim{\'e}nez-Vicente}, J. and 
	{Cardiel}, N. and {Cenarro}, A.~J. and {Falc{\'o}n-Barroso}, J. and 
	{Gorgas}, J. and {Selam}, S. and {Vazdekis}, A.},
    title = "{Medium-resolution Isaac Newton Telescope library of empirical spectra}",
  journal = {\mnras},
   eprint = {astro-ph/0607009},
 keywords = {atlases: stars: fundamental parameters: galaxies: stellar content, atlases, stars: fundamental parameters, galaxies: stellar content},
     year = 2006,
    month = sep,
   volume = 371,
    pages = {703-718},
      doi = {10.1111/j.1365-2966.2006.10699.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371..703S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{falcon2011,
   author = {{Falc{\'o}n-Barroso}, J. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Vazdekis}, A. and {Ricciardelli}, E. and {Cardiel}, N. and 
	{Cenarro}, A.~J. and {Gorgas}, J. and {Peletier}, R.~F.},
    title = "{An updated MILES stellar library and stellar population models}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.2303},
 keywords = {catalogs, methods: data analysis, techniques: spectroscopic, stars: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201116842},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A..95F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cappellari2003,
   author = {{Cappellari}, M. and {Copin}, Y.},
    title = "{Adaptive spatial binning of integral-field spectroscopic data using Voronoi tessellations}",
  journal = {\mnras},
   eprint = {astro-ph/0302262},
 keywords = {methods: data analysis, techniques: photometric, techniques: spectroscopic},
     year = 2003,
    month = jun,
   volume = 342,
    pages = {345-354},
      doi = {10.1046/j.1365-8711.2003.06541.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..345C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{krajnovic2006,
   author = {{Krajnovi{\'c}}, D. and {Cappellari}, M. and {de Zeeuw}, P.~T. and 
	{Copin}, Y.},
    title = "{Kinemetry: a generalization of photometry to the higher moments of the line-of-sight velocity distribution}",
  journal = {\mnras},
   eprint = {astro-ph/0512200},
 keywords = {methods: data analysis, techniques: photometric, techniques: spectroscopic, galaxies: kinematics and dynamics, galaxies: photometry},
     year = 2006,
    month = mar,
   volume = 366,
    pages = {787-802},
      doi = {10.1111/j.1365-2966.2005.09902.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.366..787K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yan2016spec,
   author = {{Yan}, R. and {Tremonti}, C. and {Bershady}, M.~A. and {Law}, D.~R. and 
	{Schlegel}, D.~J. and {Bundy}, K. and {Drory}, N. and {MacDonald}, N. and 
	{Bizyaev}, D. and {Blanc}, G.~A. and {Blanton}, M.~R. and {Cherinka}, B. and 
	{Eigenbrot}, A. and {Gunn}, J.~E. and {Harding}, P. and {Hogg}, D.~W. and 
	{S{\'a}nchez-Gallego}, J.~R. and {S{\'a}nchez}, S.~F. and {Wake}, D.~A. and 
	{Weijmans}, A.-M. and {Xiao}, T. and {Zhang}, K.},
    title = "{SDSS-IV/MaNGA: Spectrophotometric Calibration Technique}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1511.01496},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, methods: observational, surveys, techniques: imaging spectroscopy},
     year = 2016,
    month = jan,
   volume = 151,
      eid = {8},
    pages = {8},
      doi = {10.3847/0004-6256/151/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....151....8Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{willett2013,
       author = {{Willett}, Kyle W. and {Lintott}, Chris J. and {Bamford}, Steven P. and
         {Masters}, Karen L. and {Simmons}, Brooke D. and
         {Casteels}, Kevin R.~V. and {Edmondson}, Edward M. and
         {Fortson}, Lucy F. and {Kaviraj}, Sugata and {Keel}, William C. and
         {Melvin}, Thomas and {Nichol}, Robert C. and {Raddick}, M. Jordan and
         {Schawinski}, Kevin and {Simpson}, Robert J. and {Skibba}, Ramin A. and
         {Smith}, Arfon M. and {Thomas}, Daniel},
        title = "{Galaxy Zoo 2: detailed morphological classifications for 304 122 galaxies from the Sloan Digital Sky Survey}",
      journal = {\mnras},
     keywords = {methods: data analysis, catalogues, galaxies: elliptical and lenticular, galaxies: general, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Nov",
       volume = {435},
       number = {4},
        pages = {2835-2860},
          doi = {10.1093/mnras/stt1458},
archivePrefix = {arXiv},
       eprint = {1308.3496},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.2835W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lim2017,
       author = {{Lim}, S.~H. and {Mo}, H.~J. and {Lu}, Yi and {Wang}, Huiyuan and
         {Yang}, Xiaohu},
        title = "{Galaxy groups in the low-redshift Universe}",
      journal = {\mnras},
     keywords = {methods: statistical, galaxies: evolution, galaxies: formation, galaxies: haloes, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Sep",
       volume = {470},
       number = {3},
        pages = {2982-3005},
          doi = {10.1093/mnras/stx1462},
archivePrefix = {arXiv},
       eprint = {1706.02307},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.2982L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yang2005,
       author = {{Yang}, Xiaohu and {Mo}, H.~J. and {van den Bosch}, Frank C. and
         {Jing}, Y.~P.},
        title = "{A halo-based galaxy group finder: calibration and application to the 2dFGRS}",
      journal = {\mnras},
     keywords = {methods: statistical, galaxies: haloes, dark matter, large-scale structure of the Universe, Astrophysics},
         year = "2005",
        month = "Feb",
       volume = {356},
       number = {4},
        pages = {1293-1307},
          doi = {10.1111/j.1365-2966.2005.08560.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405234},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.356.1293Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yang2007,
       author = {{Yang}, Xiaohu and {Mo}, H.~J. and {van den Bosch}, Frank C. and
         {Pasquali}, Anna and {Li}, Cheng and {Barden}, Marco},
        title = "{Galaxy Groups in the SDSS DR4. I. The Catalog and Basic Properties}",
      journal = {\apj},
     keywords = {Cosmology: Dark Matter, Galaxies: Halos, Cosmology: Large-Scale Structure of Universe, Methods: Statistical, Astrophysics},
         year = "2007",
        month = "Dec",
       volume = {671},
       number = {1},
        pages = {153-170},
          doi = {10.1086/522027},
archivePrefix = {arXiv},
       eprint = {0707.4640},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...671..153Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pipe3Da,
   author = {{S{\'a}nchez}, S.~F. and {P{\'e}rez}, E. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Garc{\'{\i}}a-Benito}, R. and {Ibarra-Mede}, H.~J. and {Gonz{\'a}lez}, J.~J. and 
	{Rosales-Ortega}, F.~F. and {S{\'a}nchez-Menguiano}, L. and 
	{Ascasibar}, Y. and {Bitsakis}, T. and {Law}, D. and {Cano-D{\'{\i}}az}, M. and 
	{L{\'o}pez-Cob{\'a}}, C. and {Marino}, R.~A. and {Gil de Paz}, A. and 
	{L{\'o}pez-S{\'a}nchez}, A.~R. and {Barrera-Ballesteros}, J. and 
	{Galbany}, L. and {Mast}, D. and {Abril-Melgarejo}, V. and {Roman-Lopes}, A.
	},
    title = "{Pipe3D, a pipeline to analyze Integral Field Spectroscopy Data: II. Analysis sequence and CALIFA dataproducts}",
  journal = {\rmxaa},
archivePrefix = "arXiv",
   eprint = {1602.01830},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: structure, methods: data analysis, surveys, techniques: spectroscopic},
     year = 2016,
    month = apr,
   volume = 52,
    pages = {171-220},
   adsurl = {http://adsabs.harvard.edu/abs/2016RMxAA..52..171S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pipe3Dvac,
       author = {{S{\'a}nchez}, S.~F. and {Avila-Reese}, V. and {Hernandez-Toledo}, H. and
         {Cortes-Su{\'a}rez}, E. and {Rodr{\'\i}guez-Puebla}, A. and
         {Ibarra-Medel}, H. and {Cano-D{\'\i}az}, M. and
         {Barrera-Ballesteros}, J.~K. and {Negrete}, C.~A. and {Calette}, A.~R. and
         {de Lorenzo-C{\'a}ceres}, A. and {Ortega-Minakata}, R.~A. and
         {Aquino}, E. and {Valenzuela}, O. and {Clemente}, J.~C. and
         {Storchi-Bergmann}, T. and {Riffel}, R. and {Schimoia}, J. and
         {Riffel}, R.~A. and {Rembold}, S.~B. and {Brownstein}, J.~R. and
         {Pan}, K. and {Yates}, R. and {Mallmann}, N. and {Bitsakis}, T.},
        title = "{SDSS IV MaNGA - Properties of AGN Host Galaxies}",
      journal = {\rmxaa},
     keywords = {catalogues, galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: star formation, techniques: imaging spectroscopy, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {54},
        pages = {217-260},
archivePrefix = {arXiv},
       eprint = {1709.05438},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RMxAA..54..217S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{graham2018,
       author = {{Graham}, Mark T. and {Cappellari}, Michele and {Li}, Hongyu and
         {Mao}, Shude and {Bershady}, Matthew A. and {Bizyaev}, Dmitry and
         {Brinkmann}, Jonathan and {Brownstein}, Joel R. and {Bundy}, Kevin and
         {Drory}, Niv and {Law}, David R. and {Pan}, Kaike and {Thomas}, Daniel and
         {Wake}, David A. and {Weijmans}, Anne-Marie and {Westfall}, Kyle B. and
         {Yan}, Renbin},
        title = "{SDSS-IV MaNGA: stellar angular momentum of about 2300 galaxies: unveiling the bimodality of massive galaxy properties}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Jul",
       volume = {477},
       number = {4},
        pages = {4711-4737},
          doi = {10.1093/mnras/sty504},
archivePrefix = {arXiv},
       eprint = {1802.08213},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.4711G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cortese2016,
       author = {{Cortese}, L. and {Fogarty}, L.~M.~R. and {Bekki}, K. and {van de Sand
        e}, J. and {Couch}, W. and {Catinella}, B. and {Colless}, M. and
         {Obreschkow}, D. and {Taranu}, D. and {Tescari}, E. and {Barat}, D. and
         {Bland-Hawthorn}, J. and {Bloom}, J. and {Bryant}, J.~J. and
         {Cluver}, M. and {Croom}, S.~M. and {Drinkwater}, M.~J. and
         {d'Eugenio}, F. and {Konstantopoulos}, I.~S. and {Lopez-Sanchez}, A. and
         {Mahajan}, S. and {Scott}, N. and {Tonini}, C. and {Wong}, O.~I. and
         {Allen}, J.~T. and {Brough}, S. and {Goodwin}, M. and {Green}, A.~W. and
         {Ho}, I. -T. and {Kelvin}, L.~S. and {Lawrence}, J.~S. and
         {Lorente}, N.~P.~F. and {Medling}, A.~M. and {Owers}, M.~S. and
         {Richards}, S. and {Sharp}, R. and {Sweet}, S.~M.},
        title = "{The SAMI Galaxy Survey: the link between angular momentum and optical morphology}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Nov",
       volume = {463},
       number = {1},
        pages = {170-184},
          doi = {10.1093/mnras/stw1891},
archivePrefix = {arXiv},
       eprint = {1608.00291},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463..170C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pillepich18b,
       author = {{Pillepich}, Annalisa and {Nelson}, Dylan and {Hernquist}, Lars and
        {Springel}, Volker and {Pakmor}, R{\"u}diger and {Torrey}, Paul
        and {Weinberger}, Rainer and {Genel}, Shy and {Naiman}, Jill P.
        and {Marinacci}, Federico and {Vogelsberger}, Mark},
        title = "{First results from the IllustrisTNG simulations: the stellar mass content of groups and clusters of galaxies}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: clusters: general, galaxies: general, galaxies: groups: general, cosmology: theory, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = Mar,
       volume = {475},
        pages = {648-675},
          doi = {10.1093/mnras/stx3112},
archivePrefix = {arXiv},
       eprint = {1707.03406},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.475..648P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{springel18,
       author = {{Springel}, Volker and {Pakmor}, R{\"u}diger and {Pillepich}, Annalisa
        and {Weinberger}, Rainer and {Nelson}, Dylan and {Hernquist},
        Lars and {Vogelsberger}, Mark and {Genel}, Shy and {Torrey},
        Paul and {Marinacci}, Federico and {Naiman}, Jill},
        title = "{First results from the IllustrisTNG simulations: matter and galaxy clustering}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxy formation, large-scale structure of Universe, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = Mar,
       volume = {475},
        pages = {676-698},
          doi = {10.1093/mnras/stx3304},
archivePrefix = {arXiv},
       eprint = {1707.03397},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.475..676S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nelson18,
       author = {{Nelson}, Dylan and {Pillepich}, Annalisa and {Springel}, Volker and
        {Weinberger}, Rainer and {Hernquist}, Lars and {Pakmor},
        R{\"u}diger and {Genel}, Shy and {Torrey}, Paul and
        {Vogelsberger}, Mark and {Kauffmann}, Guinevere and {Marinacci},
        Federico and {Naiman}, Jill},
        title = "{First results from the IllustrisTNG simulations: the galaxy colour bimodality}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = Mar,
       volume = {475},
        pages = {624-647},
          doi = {10.1093/mnras/stx3040},
archivePrefix = {arXiv},
       eprint = {1707.03395},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.475..624N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naiman18,
       author = {{Naiman}, Jill P. and {Pillepich}, Annalisa and {Springel}, Volker and
        {Ramirez-Ruiz}, Enrico and {Torrey}, Paul and {Vogelsberger},
        Mark and {Pakmor}, R{\"u}diger and {Nelson}, Dylan and
        {Marinacci}, Federico and {Hernquist}, Lars and {Weinberger},
        Rainer and {Genel}, Shy},
        title = "{First results from the IllustrisTNG simulations: a tale of two elements - chemical evolution of magnesium and europium}",
      journal = {\mnras},
     keywords = {methods: numerical, Galaxy: formation, cosmology: theory, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = Jun,
       volume = {477},
        pages = {1206-1224},
          doi = {10.1093/mnras/sty618},
archivePrefix = {arXiv},
       eprint = {1707.03401},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.477.1206N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{marinacci18,
       author = {{Marinacci}, Federico and {Vogelsberger}, Mark and {Pakmor}, R{\"u}diger
        and {Torrey}, Paul and {Springel}, Volker and {Hernquist}, Lars
        and {Nelson}, Dylan and {Weinberger}, Rainer and {Pillepich},
        Annalisa and {Naiman}, Jill and {Genel}, Shy},
        title = "{First results from the IllustrisTNG simulations: radio haloes and magnetic fields}",
      journal = {\mnras},
     keywords = {magnetic fields, MHD, methods: numerical, galaxies: clusters: general, cosmology: theory, radio continuum: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = Nov,
       volume = {480},
        pages = {5113-5139},
          doi = {10.1093/mnras/sty2206},
archivePrefix = {arXiv},
       eprint = {1707.03396},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018MNRAS.480.5113M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{springel10,
       author = {{Springel}, Volker},
        title = "{E pur si muove: Galilean-invariant cosmological hydrodynamical simulations on a moving mesh}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: interactions, cosmology: dark matter, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = Jan,
       volume = {401},
        pages = {791-851},
          doi = {10.1111/j.1365-2966.2009.15715.x},
archivePrefix = {arXiv},
       eprint = {0901.4107},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2010MNRAS.401..791S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pakmor11,
       author = {{Pakmor}, Ruediger and {Bauer}, Andreas and {Springel}, Volker},
        title = "{Magnetohydrodynamics on an unstructured moving grid}",
      journal = {\mnras},
     keywords = {MHD, turbulence, methods: numerical, stars: formation, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = Dec,
       volume = {418},
        pages = {1392-1401},
          doi = {10.1111/j.1365-2966.2011.19591.x},
archivePrefix = {arXiv},
       eprint = {1108.1792},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2011MNRAS.418.1392P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pakmor13,
   author = {{Pakmor}, R. and {Springel}, V.},
    title = "{Simulations of magnetic fields in isolated disc galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.1452},
 primaryClass = "astro-ph.CO",
 keywords = {MHD, methods: numerical, galaxies: formation},
     year = 2013,
    month = jun,
   volume = 432,
    pages = {176-193},
      doi = {10.1093/mnras/stt428},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432..176P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weinberger17,
   author = {{Weinberger}, R. and {Springel}, V. and {Hernquist}, L. and 
	{Pillepich}, A. and {Marinacci}, F. and {Pakmor}, R. and {Nelson}, D. and 
	{Genel}, S. and {Vogelsberger}, M. and {Naiman}, J. and {Torrey}, P.
	},
    title = "{Simulating galaxy formation with black hole driven thermal and kinetic feedback}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.03486},
 keywords = {black hole physics, methods: numerical, galaxies: clusters: general, galaxies: evolution, galaxies: formation, cosmology: theory},
     year = 2017,
    month = mar,
   volume = 465,
    pages = {3291-3308},
      doi = {10.1093/mnras/stw2944},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.3291W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pillepich18a,
   author = {{Pillepich}, A. and {Springel}, V. and {Nelson}, D. and {Genel}, S. and 
	{Naiman}, J. and {Pakmor}, R. and {Hernquist}, L. and {Torrey}, P. and 
	{Vogelsberger}, M. and {Weinberger}, R. and {Marinacci}, F.},
    title = "{Simulating galaxy formation with the IllustrisTNG model}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1703.02970},
 keywords = {methods: numerical, galaxies: evolution, galaxies: formation},
     year = 2018,
    month = jan,
   volume = 473,
    pages = {4077-4106},
      doi = {10.1093/mnras/stx2656},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473.4077P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{davis85,
   author = {{Davis}, M. and {Efstathiou}, G. and {Frenk}, C.~S. and {White}, S.~D.~M.
	},
    title = "{The evolution of large-scale structure in a universe dominated by cold dark matter}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Cosmology, Galactic Clusters, Galactic Evolution, Missing Mass (Astrophysics), Weak Interactions (Field Theory), Astronomical Models, Computerized Simulation, Correlation, Many Body Problem, Mass Distribution, Mass To Light Ratios, Matter (Physics), Radial Velocity, Red Shift},
     year = 1985,
    month = may,
   volume = 292,
    pages = {371-394},
      doi = {10.1086/163168},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...292..371D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{springel01,
   author = {{Springel}, V. and {White}, S.~D.~M. and {Tormen}, G. and {Kauffmann}, G.
	},
    title = "{Populating a cluster of galaxies - I. Results at [formmu2]z=0}",
  journal = {\mnras},
   eprint = {astro-ph/0012055},
 keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: FORMATION, DARK MATTER},
     year = 2001,
    month = dec,
   volume = 328,
    pages = {726-750},
      doi = {10.1046/j.1365-8711.2001.04912.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.328..726S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pillepich2019,
       author = {{Pillepich}, Annalisa and {Nelson}, Dylan and {Springel}, Volker and
         {Pakmor}, Ruediger and {Torrey}, Paul and {Weinberger}, Rainer and
         {Vogelsberger}, Mark and {Marinacci}, Federico and {Genel}, Shy and
         {van der Wel}, Arjen and {Hernquist}, Lars},
        title = "{First Results from the TNG50 Simulation: The evolution of stellar and gaseous disks across cosmic time}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2019",
        month = "Feb",
          eid = {arXiv:1902.05553},
        pages = {arXiv:1902.05553},
archivePrefix = {arXiv},
       eprint = {1902.05553},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190205553P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chisari+17,
       author = {{Chisari}, N.~E. and {Koukoufilippas}, N. and {Jindal}, A. and
         {Peirani}, S. and {Beckmann}, R.~S. and {Codis}, S. and
         {Devriendt}, J. and {Miller}, L. and {Dubois}, Y. and {Laigle}, C. and
         {Slyz}, A. and {Pichon}, C.},
        title = "{Galaxy-halo alignments in the Horizon-AGN cosmological hydrodynamical simulation}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: numerical, large-scale structure of Universe, cosmology: theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2017",
        month = "Nov",
       volume = {472},
       number = {1},
        pages = {1163-1181},
          doi = {10.1093/mnras/stx1998},
archivePrefix = {arXiv},
       eprint = {1702.03913},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472.1163C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{starkenburg+19,
       author = {{Starkenburg}, Tjitske K. and {Sales}, Laura. V. and {Genel}, Shy and
         {Manzano-King}, Christina and {Canalizo}, Gabriela and
         {Hernquist}, Lars},
        title = "{On the Origin of Star─Gas Counterrotation in Low-mass Galaxies}",
      journal = {\apj},
     keywords = {galaxies: dwarf, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jun",
       volume = {878},
       number = {2},
          eid = {143},
        pages = {143},
          doi = {10.3847/1538-4357/ab2128},
archivePrefix = {arXiv},
       eprint = {1903.03627},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...878..143S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chen2016,
       author = {{Chen}, Yan-Mei and {Shi}, Yong and {Tremonti}, Christy A. and
        {Bershady}, Matt and {Merrifield}, Michael and {Emsellem}, Eric
        and {Jin}, Yi-Fei and {Huang}, Song and {Fu}, Hai and {Wake},
        David A. and {Bundy}, Kevin and {Stark}, David and {Lin}, Lihwai
        and {Argudo-Fernandez}, Maria and {Bergmann}, Thaisa Storchi and
        {Bizyaev}, Dmitry and {Brownstein}, Joel and {Bureau}, Martin
        and {Chisholm}, John and {Drory}, Niv and {Guo}, Qi and {Hao},
        Lei and {Hu}, Jian and {Li}, Cheng and {Li}, Ran and {Roman
        Lopes}, Alexandre and {Pan}, Kai-Ke and {Riffel}, Rogemar A. and
        {Thomas}, Daniel and {Wang}, Lan and {Westfall}, Kyle and {Yan},
        Ren-Bin},
        title = "{The growth of the central region by acquisition of counterrotating gas
        in star-forming galaxies}",
      journal = {Nature Communications},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = Oct,
       volume = {7},
          doi = {10.1038/ncomms13269},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016NatCo...713269C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jin2016,
       author = {{Jin}, Yifei and {Chen}, Yanmei and {Shi}, Yong and {Tremonti}, C.~A. and
         {Bershady}, M.~A. and {Merrifield}, M. and {Emsellem}, E. and
         {Fu}, Hai and {Wake}, D. and {Bundy}, K. and {Lin}, Lihwai and
         {Argudo-Fernandez}, M. and {Huang}, Song and {Stark}, D.~V. and
         {Storchi-Bergmann}, T. and {Bizyaev}, D. and {Brownstein}, J. and
         {Chisholm}, J. and {Guo}, Qi and {Hao}, Lei and {Hu}, Jian and
         {Li}, Cheng and {Li}, Ran and {Masters}, K.~L. and {Malanushenko}, E. and
         {Pan}, Kaike and {Riffel}, R.~A. and {Roman-Lopes}, A. and
         {Simmons}, A. and {Thomas}, D. and {Wang}, Lan and {Westfall}, K. and
         {Yan}, Renbin},
        title = "{SDSS-IV MaNGA: properties of galaxies with kinematically decoupled stellar and gaseous components}",
      journal = {\mnras},
     keywords = {Galaxy: abundances, galaxies: evolution, galaxies: formation, galaxies: stellar content, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Nov",
       volume = {463},
       number = {1},
        pages = {913-926},
          doi = {10.1093/mnras/stw2055},
archivePrefix = {arXiv},
       eprint = {1611.00528},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463..913J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{roy2018,
       author = {{Roy}, Namrata and {Bundy}, Kevin and {Cheung}, Edmond and {MaNGA Team}},
        title = "{Red Geyser: A New Class of Galaxy with Large-scale AGN-driven Winds}",
    booktitle = {American Astronomical Society Meeting Abstracts \#231},
         year = "2018",
       series = {American Astronomical Society Meeting Abstracts},
       volume = {231},
        month = "Jan",
          eid = {250.46},
        pages = {250.46},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AAS...23125046R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peebles1969,
       author = {{Peebles}, P.~J.~E.},
        title = "{Origin of the Angular Momentum of Galaxies}",
      journal = {\apj},
         year = "1969",
        month = "Feb",
       volume = {155},
        pages = {393},
          doi = {10.1086/149876},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969ApJ...155..393P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Doroshkevich1970,
       author = {{Doroshkevich}, A.~G.},
        title = "{Spatial structure of perturbations and origin of galactic rotation in fluctuation theory}",
      journal = {Astrophysics},
         year = "1970",
        month = "Oct",
       volume = {6},
       number = {4},
        pages = {320-330},
          doi = {10.1007/BF01001625},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970Ap......6..320D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lagos2017,
       author = {{Lagos}, Claudia del P. and {Theuns}, Tom and {Stevens}, Adam R.~H. and
         {Cortese}, Luca and {Padilla}, Nelson D. and {Davis}, Timothy A. and
         {Contreras}, Sergio and {Croton}, Darren},
        title = "{Angular momentum evolution of galaxies in EAGLE}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Feb",
       volume = {464},
       number = {4},
        pages = {3850-3870},
          doi = {10.1093/mnras/stw2610},
archivePrefix = {arXiv},
       eprint = {1609.01739},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.464.3850L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lagos2018,
       author = {{Lagos}, Claudia del P. and {Stevens}, Adam R.~H. and
         {Bower}, Richard G. and {Davis}, Timothy A. and {Contreras}, Sergio and
         {Padilla}, Nelson D. and {Obreschkow}, Danail and {Croton}, Darren and
         {Trayford}, James W. and {Welker}, Charlotte and {Theuns}, Tom},
        title = "{Quantifying the impact of mergers on the angular momentum of simulated galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Feb",
       volume = {473},
       number = {4},
        pages = {4956-4974},
          doi = {10.1093/mnras/stx2667},
archivePrefix = {arXiv},
       eprint = {1701.04407},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.4956L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{genel2015,
       author = {{Genel}, Shy and {Fall}, S. Michael and {Hernquist}, Lars and
         {Vogelsberger}, Mark and {Snyder}, Gregory F. and
         {Rodriguez-Gomez}, Vicente and {Sijacki}, Debora and {Springel}, Volker},
        title = "{Galactic Angular Momentum in the Illustris Simulation: Feedback and the Hubble Sequence}",
      journal = {\apjl},
     keywords = {galaxies: formation, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: structure, hydrodynamics, methods: numerical, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "May",
       volume = {804},
       number = {2},
          eid = {L40},
        pages = {L40},
          doi = {10.1088/2041-8205/804/2/L40},
archivePrefix = {arXiv},
       eprint = {1503.01117},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...804L..40G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeFelippis2017,
       author = {{DeFelippis}, Daniel and {Genel}, Shy and {Bryan}, Greg L. and
         {Fall}, S. Michael},
        title = "{The Impact of Galactic Winds on the Angular Momentum of Disk Galaxies in the Illustris Simulation}",
      journal = {\apj},
     keywords = {galaxies: formation, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: structure, hydrodynamics, methods: numerical, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "May",
       volume = {841},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/1538-4357/aa6dfc},
archivePrefix = {arXiv},
       eprint = {1703.03806},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841...16D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fall1980,
       author = {{Fall}, S.~M. and {Efstathiou}, G.},
        title = "{Formation and rotation of disc galaxies with haloes.}",
      journal = {\mnras},
     keywords = {Disk Galaxies, Galactic Evolution, Galactic Rotation, Galactic Structure, Halos, Angular Momentum, Astronomical Models, Interstellar Gas, Mass Ratios, Astrophysics},
         year = "1980",
        month = "Oct",
       volume = {193},
        pages = {189-206},
          doi = {10.1093/mnras/193.2.189},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980MNRAS.193..189F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mo1998,
       author = {{Mo}, H.~J. and {Mao}, Shude and {White}, Simon D.~M.},
        title = "{The formation of galactic discs}",
      journal = {\mnras},
     keywords = {GALAXIES: FORMATION, GALAXIES: SPIRAL, GALAXIES: STRUCTURE, COSMOLOGY: THEORY, DARK MATTER, Astrophysics},
         year = "1998",
        month = "Apr",
       volume = {295},
       number = {2},
        pages = {319-336},
          doi = {10.1046/j.1365-8711.1998.01227.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/9707093},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998MNRAS.295..319M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{hoyle1951,
       author = {{Hoyle}, F.},
        title = "{The Origin of the Rotations of the Galaxies}",
    booktitle = {Problems of Cosmical Aerodynamics},
         year = "1951",
        month = "Jan",
        pages = {195},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1951pca..conf..195H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{white1978,
       author = {{White}, S.~D.~M. and {Rees}, M.~J.},
        title = "{Core condensation in heavy halos: a two-stage theory for galaxy formation and clustering.}",
      journal = {\mnras},
     keywords = {Astronomical Models, Galactic Clusters, Galactic Evolution, Galactic Nuclei, Gravitational Effects, Halos, Critical Mass, Dark Matter, Dynamic Models, Interstellar Gas, Luminosity, Many Body Problem, Red Shift, Astrophysics, Formation:Galaxies},
         year = "1978",
        month = "May",
       volume = {183},
        pages = {341-358},
          doi = {10.1093/mnras/183.3.341},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978MNRAS.183..341W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{scannapieco2009,
       author = {{Scannapieco}, Cecilia and {White}, Simon D.~M. and {Springel}, Volker and
         {Tissera}, Patricia B.},
        title = "{The formation and survival of discs in a {\ensuremath{\Lambda}}CDM universe}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: formation, cosmology: theory, Astrophysics},
         year = "2009",
        month = "Jun",
       volume = {396},
       number = {2},
        pages = {696-708},
          doi = {10.1111/j.1365-2966.2009.14764.x},
archivePrefix = {arXiv},
       eprint = {0812.0976},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.396..696S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zavala2008,
       author = {{Zavala}, Jesus and {Okamoto}, Takashi and {Frenk}, Carlos S.},
        title = "{Bulges versus discs: the evolution of angular momentum in cosmological simulations of galaxy formation}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: evolution, galaxies: formation, Astrophysics},
         year = "2008",
        month = "Jun",
       volume = {387},
       number = {1},
        pages = {364-370},
          doi = {10.1111/j.1365-2966.2008.13243.x},
archivePrefix = {arXiv},
       eprint = {0710.2901},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.387..364Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{emsellem2007,
       author = {{Emsellem}, Eric and {Cappellari}, Michele and {Krajnovi{\'c}}, Davor and
         {van de Ven}, Glenn and {Bacon}, R. and {Bureau}, M. and
         {Davies}, Roger L. and {de Zeeuw}, P.~T. and
         {Falc{\'o}n-Barroso}, Jes{\'u}s and {Kuntschner}, Harald and
         {McDermid}, Richard and {Peletier}, Reynier F. and {Sarzi}, Marc},
        title = "{The SAURON project - IX. A kinematic classification for early-type galaxies}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics},
         year = "2007",
        month = "Aug",
       volume = {379},
       number = {2},
        pages = {401-417},
          doi = {10.1111/j.1365-2966.2007.11752.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703531},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.379..401E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sauron,
       author = {{Bacon}, R. and {Copin}, Y. and {Monnet}, G. and {Miller}, Bryan W. and
         {Allington-Smith}, J.~R. and {Bureau}, M. and {Carollo}, C.~M. and
         {Davies}, Roger L. and {Emsellem}, Eric and {Kuntschner}, Harald and
         {Peletier}, Reynier F. and {Verolme}, E.~K. and {de Zeeuw}, P. Tim},
        title = "{The SAURON project - I. The panoramic integral-field spectrograph}",
      journal = {\mnras},
     keywords = {INSTRUMENTATION: SPECTROGRAPHS, GALAXIES: ELLIPTICAL AND LENTICULAR, CD, GALAXIES: INDIVIDUAL: NGC 3377, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = "2001",
        month = "Sep",
       volume = {326},
       number = {1},
        pages = {23-35},
          doi = {10.1046/j.1365-8711.2001.04612.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103451},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.326...23B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{atlas3d,
       author = {{Cappellari}, Michele and {Emsellem}, Eric and {Krajnovi{\'c}}, Davor and
         {McDermid}, Richard M. and {Scott}, Nicholas and
         {Verdoes Kleijn}, G.~A. and {Young}, Lisa M. and {Alatalo}, Katherine and
         {Bacon}, R. and {Blitz}, Leo and {Bois}, Maxime and
         {Bournaud}, Fr{\'e}d{\'e}ric and {Bureau}, M. and {Davies}, Roger L. and
         {Davis}, Timothy A. and {de Zeeuw}, P.~T. and {Duc}, Pierre-Alain and
         {Khochfar}, Sadegh and {Kuntschner}, Harald and
         {Lablanche}, Pierre-Yves and {Morganti}, Raffaella and
         {Naab}, Thorsten and {Oosterloo}, Tom and {Sarzi}, Marc and
         {Serra}, Paolo and {Weijmans}, Anne-Marie},
        title = "{The ATLAS$^{3D}$ project - I. A volume-limited sample of 260 nearby early-type galaxies: science goals and selection criteria}",
      journal = {\mnras},
     keywords = {galaxies: distances and redshifts, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "May",
       volume = {413},
       number = {2},
        pages = {813-836},
          doi = {10.1111/j.1365-2966.2010.18174.x},
archivePrefix = {arXiv},
       eprint = {1012.1551},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.413..813C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{emsellem2011,
       author = {{Emsellem}, Eric and {Cappellari}, Michele and {Krajnovi{\'c}}, Davor and
         {Alatalo}, Katherine and {Blitz}, Leo and {Bois}, Maxime and
         {Bournaud}, Fr{\'e}d{\'e}ric and {Bureau}, Martin and
         {Davies}, Roger L. and {Davis}, Timothy A. and {de Zeeuw}, P.~T. and
         {Khochfar}, Sadegh and {Kuntschner}, Harald and
         {Lablanche}, Pierre-Yves and {McDermid}, Richard M. and
         {Morganti}, Raffaella and {Naab}, Thorsten and {Oosterloo}, Tom and
         {Sarzi}, Marc and {Scott}, Nicholas and {Serra}, Paolo and
         {van de Ven}, Glenn and {Weijmans}, Anne-Marie and {Young}, Lisa M.},
        title = "{The ATLAS$^{3D}$ project - III. A census of the stellar angular momentum within the effective radius of early-type galaxies: unveiling the distribution of fast and slow rotators}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Jun",
       volume = {414},
       number = {2},
        pages = {888-912},
          doi = {10.1111/j.1365-2966.2011.18496.x},
archivePrefix = {arXiv},
       eprint = {1102.4444},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.414..888E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{arnold2014,
       author = {{Arnold}, Jacob A. and {Romanowsky}, Aaron J. and {Brodie}, Jean P. and
         {Forbes}, Duncan A. and {Strader}, Jay and {Spitler}, Lee R. and
         {Foster}, Caroline and {Blom}, Christina and {Kartha}, Sreeja S. and
         {Pastorello}, Nicola and {Pota}, Vincenzo and {Usher}, Christopher and
         {Woodley}, Kristin A.},
        title = "{The SLUGGS Survey: Wide-field Stellar Kinematics of Early-type Galaxies}",
      journal = {\apj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: halos, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Aug",
       volume = {791},
       number = {2},
          eid = {80},
        pages = {80},
          doi = {10.1088/0004-637X/791/2/80},
archivePrefix = {arXiv},
       eprint = {1310.2607},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...791...80A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{foster2013,
       author = {{Foster}, Caroline and {Arnold}, Jacob A. and {Forbes}, Duncan A. and
         {Pastorello}, Nicola and {Romanowsky}, Aaron J. and {Spitler}, Lee R. and
         {Strader}, Jay and {Brodie}, Jean P.},
        title = "{The SLUGGS survey: outer triaxiality of the fast rotator elliptical NGC 4473}",
      journal = {\mnras},
     keywords = {galaxies: haloes, galaxies: individual: (NGC 4473), galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Nov",
       volume = {435},
       number = {4},
        pages = {3587-3591},
          doi = {10.1093/mnras/stt1550},
archivePrefix = {arXiv},
       eprint = {1308.3531},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.3587F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{croom2012,
   author = {{Croom}, S.~M. and {Lawrence}, J.~S. and {Bland-Hawthorn}, J. and 
	{Bryant}, J.~J. and {Fogarty}, L. and {Richards}, S. and {Goodwin}, M. and 
	{Farrell}, T. and {Miziarski}, S. and {Heald}, R. and {Jones}, D.~H. and 
	{Lee}, S. and {Colless}, M. and {Brough}, S. and {Hopkins}, A.~M. and 
	{Bauer}, A.~E. and {Birchall}, M.~N. and {Ellis}, S. and {Horton}, A. and 
	{Leon-Saval}, S. and {Lewis}, G. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Min}, S.-S. and {Trinh}, C. and {Trowland}, H.},
    title = "{The Sydney-AAO Multi-object Integral field spectrograph}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1112.3367},
 keywords = {instrumentation: spectrographs, techniques: imaging spectroscopy, surveys, galaxies: general, galaxies: kinematics and dynamics},
     year = 2012,
    month = mar,
   volume = 421,
    pages = {872-893},
      doi = {10.1111/j.1365-2966.2011.20365.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421..872C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bryant2015,
   author = {{Bryant}, J.~J. and {Owers}, M.~S. and {Robotham}, A.~S.~G. and 
	{Croom}, S.~M. and {Driver}, S.~P. and {Drinkwater}, M.~J. and 
	{Lorente}, N.~P.~F. and {Cortese}, L. and {Scott}, N. and {Colless}, M. and 
	{Schaefer}, A. and {Taylor}, E.~N. and {Konstantopoulos}, I.~S. and 
	{Allen}, J.~T. and {Baldry}, I. and {Barnes}, L. and {Bauer}, A.~E. and 
	{Bland-Hawthorn}, J. and {Bloom}, J.~V. and {Brooks}, A.~M. and 
	{Brough}, S. and {Cecil}, G. and {Couch}, W. and {Croton}, D. and 
	{Davies}, R. and {Ellis}, S. and {Fogarty}, L.~M.~R. and {Foster}, C. and 
	{Glazebrook}, K. and {Goodwin}, M. and {Green}, A. and {Gunawardhana}, M.~L. and 
	{Hampton}, E. and {Ho}, I.-T. and {Hopkins}, A.~M. and {Kewley}, L. and 
	{Lawrence}, J.~S. and {Leon-Saval}, S.~G. and {Leslie}, S. and 
	{McElroy}, R. and {Lewis}, G. and {Liske}, J. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Mahajan}, S. and {Medling}, A.~M. and {Metcalfe}, N. and {Meyer}, M. and 
	{Mould}, J. and {Obreschkow}, D. and {O'Toole}, S. and {Pracy}, M. and 
	{Richards}, S.~N. and {Shanks}, T. and {Sharp}, R. and {Sweet}, S.~M. and 
	{Thomas}, A.~D. and {Tonini}, C. and {Walcher}, C.~J.},
    title = "{The SAMI Galaxy Survey: instrument specification and target selection}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1407.7335},
 keywords = {instrumentation: miscellaneous, instrumentation: spectrographs, techniques: imaging spectroscopy, surveys, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2015,
    month = mar,
   volume = 447,
    pages = {2857-2879},
      doi = {10.1093/mnras/stu2635},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.2857B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bundy2015,
   author = {{Bundy}, K. and {Bershady}, M.~A. and {Law}, D.~R. and {Yan}, R. and 
	{Drory}, N. and {MacDonald}, N. and {Wake}, D.~A. and {Cherinka}, B. and 
	{S{\'a}nchez-Gallego}, J.~R. and {Weijmans}, A.-M. and {Thomas}, D. and 
	{Tremonti}, C. and {Masters}, K. and {Coccato}, L. and {Diamond-Stanic}, A.~M. and 
	{Arag{\'o}n-Salamanca}, A. and {Avila-Reese}, V. and {Badenes}, C. and 
	{Falc{\'o}n-Barroso}, J. and {Belfiore}, F. and {Bizyaev}, D. and 
	{Blanc}, G.~A. and {Bland-Hawthorn}, J. and {Blanton}, M.~R. and 
	{Brownstein}, J.~R. and {Byler}, N. and {Cappellari}, M. and 
	{Conroy}, C. and {Dutton}, A.~A. and {Emsellem}, E. and {Etherington}, J. and 
	{Frinchaboy}, P.~M. and {Fu}, H. and {Gunn}, J.~E. and {Harding}, P. and 
	{Johnston}, E.~J. and {Kauffmann}, G. and {Kinemuchi}, K. and 
	{Klaene}, M.~A. and {Knapen}, J.~H. and {Leauthaud}, A. and 
	{Li}, C. and {Lin}, L. and {Maiolino}, R. and {Malanushenko}, V. and 
	{Malanushenko}, E. and {Mao}, S. and {Maraston}, C. and {McDermid}, R.~M. and 
	{Merrifield}, M.~R. and {Nichol}, R.~C. and {Oravetz}, D. and 
	{Pan}, K. and {Parejko}, J.~K. and {Sanchez}, S.~F. and {Schlegel}, D. and 
	{Simmons}, A. and {Steele}, O. and {Steinmetz}, M. and {Thanjavur}, K. and 
	{Thompson}, B.~A. and {Tinker}, J.~L. and {van den Bosch}, R.~C.~E. and 
	{Westfall}, K.~B. and {Wilkinson}, D. and {Wright}, S. and {Xiao}, T. and 
	{Zhang}, K.},
    title = "{Overview of the SDSS-IV MaNGA Survey: Mapping nearby Galaxies at Apache Point Observatory}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1412.1482},
 keywords = {galaxies: evolution, galaxies: general, surveys, techniques: imaging spectroscopy},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {7},
    pages = {7},
      doi = {10.1088/0004-637X/798/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blanton2017,
   author = {{Blanton}, M.~R. and {Bershady}, M.~A. and {Abolfathi}, B. and 
	{Albareti}, F.~D. and {Allende Prieto}, C. and {Almeida}, A. and 
	{Alonso-Garc{\'{\i}}a}, J. and {Anders}, F. and {Anderson}, S.~F. and 
	{Andrews}, B. and et al.},
    title = "{Sloan Digital Sky Survey IV: Mapping the Milky Way, Nearby Galaxies, and the Distant Universe}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1703.00052},
 keywords = {cosmology: observations, galaxies: general, Galaxy: general, instrumentation: spectrographs, stars: general, surveys},
     year = 2017,
    month = jul,
   volume = 154,
      eid = {28},
    pages = {28},
      doi = {10.3847/1538-3881/aa7567},
   adsurl = {http://adsabs.harvard.edu/abs/2017AJ....154...28B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{duckworth2019,
       author = {{Duckworth}, Christopher and {Tojeiro}, Rita and {Kraljic}, Katarina and
         {Sgr{\'o}}, Mario A. and {Wild}, Vivienne and {Weijmans}, Anne-Marie and
         {Lacerna}, Ivan and {Drory}, Niv},
        title = "{SDSS-IV MaNGA: signatures of halo assembly in kinematically misaligned galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: haloes, galaxies: kinematics and dynamics, dark matter, large-scale structure of Universe, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Feb",
       volume = {483},
       number = {1},
        pages = {172-188},
          doi = {10.1093/mnras/sty3101},
archivePrefix = {arXiv},
       eprint = {1811.06408},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483..172D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{davis2016,
author = {Davis, Timothy A. and Bureau, Martin},
title = {On the depletion and accretion time-scales of cold gas in local early-type galaxies},
journal = {\mnras},
volume = {457},
number = {1},
pages = {272-280},
year = {2016},
doi = {10.1093/mnras/stv2998},
URL = { + http://dx.doi.org/10.1093/mnras/stv2998},
eprint = {/oup/backfile/content_public/journal/mnras/457/1/10.1093_mnras_stv2998/2/stv2998.pdf}
}

@ARTICLE{davis2011,
   author = {{Davis}, T.~A. and {Alatalo}, K. and {Sarzi}, M. and {Bureau}, M. and 
	{Young}, L.~M. and {Blitz}, L. and {Serra}, P. and {Crocker}, A.~F. and 
	{Krajnovi{\'c}}, D. and {McDermid}, R.~M. and {Bois}, M. and 
	{Bournaud}, F. and {Cappellari}, M. and {Davies}, R.~L. and 
	{Duc}, P.-A. and {de Zeeuw}, P.~T. and {Emsellem}, E. and {Khochfar}, S. and 
	{Kuntschner}, H. and {Lablanche}, P.-Y. and {Morganti}, R. and 
	{Naab}, T. and {Oosterloo}, T. and {Scott}, N. and {Weijmans}, A.-M.
	},
    title = "{The ATLAS$^{3D}$ project - X. On the origin of the molecular and ionized gas in early-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1107.0002},
 primaryClass = "astro-ph.CO",
 keywords = {stars: mass-loss, ISM: evolution, ISM: molecules, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: ISM},
     year = 2011,
    month = oct,
   volume = 417,
    pages = {882-899},
      doi = {10.1111/j.1365-2966.2011.19355.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417..882D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vdvoort2015,
       author = {{van de Voort}, Freeke and {Davis}, Timothy A. and
         {Kere{\v{s}}}, Du{\v{s}}an and {Quataert}, Eliot and
         {Faucher-Gigu{\`e}re}, Claude-Andr{\'e} and {Hopkins}, Philip F.},
        title = "{The creation and persistence of a misaligned gas disc in a simulated early-type galaxy}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "Aug",
       volume = {451},
       number = {3},
        pages = {3269-3277},
          doi = {10.1093/mnras/stv1217},
archivePrefix = {arXiv},
       eprint = {1504.03685},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.3269V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lagos2015,
       author = {{Lagos}, Claudia del P. and {Padilla}, Nelson D. and
         {Davis}, Timothy A. and {Lacey}, Cedric G. and {Baugh}, Carlton M. and
         {Gonzalez-Perez}, Violeta and {Zwaan}, Martin A. and
         {Contreras}, Sergio},
        title = "{The origin of the atomic and molecular gas contents of early-type galaxies - II. Misaligned gas accretion}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: ISM, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Apr",
       volume = {448},
       number = {2},
        pages = {1271-1287},
          doi = {10.1093/mnras/stu2763},
archivePrefix = {arXiv},
       eprint = {1410.5437},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.448.1271L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bryant2019,
       author = {{Bryant}, J.~J. and {Croom}, S.~M. and {van de Sande}, J. and
         {Scott}, N. and {Fogarty}, L.~M.~R. and {Bland-Hawthorn}, J. and
         {Bloom}, J.~V. and {Taylor}, E.~N. and {Brough}, S. and {Robotham}, A. and
         {Cortese}, L. and {Couch}, W. and {Owers}, M.~S. and {Medling}, A.~M. and
         {Federrath}, C. and {Bekki}, K. and {Richards}, S.~N. and
         {Lawrence}, J.~S. and {Konstantopoulos}, I.~S.},
        title = "{The SAMI Galaxy Survey: stellar and gas misalignments and the origin of gas in nearby galaxies}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, surveys, galaxies: evolution, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Feb",
       volume = {483},
       number = {1},
        pages = {458-479},
          doi = {10.1093/mnras/sty3122},
archivePrefix = {arXiv},
       eprint = {1811.09298},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483..458B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{davis2011molecular,
       author = {{Davis}, Timothy A. and {Alatalo}, Katherine and {Bureau}, Martin and
         {Cappellari}, Michele and {Scott}, Nicholas and {Young}, Lisa M. and
         {Blitz}, Leo and {Crocker}, Alison and {Bayet}, Estelle and
         {Bois}, Maxime and {Bournaud}, Fr{\'e}d{\'e}ric and {Davies}, Roger L. and
         {de Zeeuw}, P.~T. and {Duc}, Pierre-Alain and {Emsellem}, Eric and
         {Khochfar}, Sadegh and {Krajnovi{\'c}}, Davor and {Kuntschner}, Harald and
         {Lablanche}, Pierre-Yves and {McDermid}, Richard M. and
         {Morganti}, Raffaella and {Naab}, Thorsten and {Oosterloo}, Tom and
         {Sarzi}, Marc and {Serra}, Paolo and {Weijmans}, Anne-Marie},
        title = "{The ATLAS$^{3D}$ Project - XIV. The extent and kinematics of the molecular gas in early-type galaxies}",
      journal = {\mnras},
     keywords = {ISM: evolution, ISM: kinematics and dynamics, ISM: molecules, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: ISM, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Feb",
       volume = {429},
       number = {1},
        pages = {534-555},
          doi = {10.1093/mnras/sts353},
archivePrefix = {arXiv},
       eprint = {1211.1011},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..534D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{genel2018,
       author = {{Genel}, Shy and {Nelson}, Dylan and {Pillepich}, Annalisa and
         {Springel}, Volker and {Pakmor}, R{\"u}diger and {Weinberger}, Rainer and
         {Hernquist}, Lars and {Naiman}, Jill and {Vogelsberger}, Mark and
         {Marinacci}, Federico and {Torrey}, Paul},
        title = "{The size evolution of star-forming and quenched galaxies in the IllustrisTNG simulation}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: evolution, galaxies: formation, galaxies: structure, cosmology: theory, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Mar",
       volume = {474},
       number = {3},
        pages = {3976-3996},
          doi = {10.1093/mnras/stx3078},
archivePrefix = {arXiv},
       eprint = {1707.05327},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474.3976G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conroy2009,
   author = {{Conroy}, C. and {Gunn}, J.~E. and {White}, M.},
    title = "{The Propagation of Uncertainties in Stellar Population Synthesis Modeling. I. The Relevance of Uncertain Aspects of Stellar Evolution and the Initial Mass Function to the Derived Physical Properties of Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.4261},
 keywords = {galaxies: evolution, galaxies: stellar content, stars: evolution},
     year = 2009,
    month = jul,
   volume = 699,
    pages = {486-506},
      doi = {10.1088/0004-637X/699/1/486},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...699..486C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conroy2010,
   author = {{Conroy}, C. and {Gunn}, J.~E.},
    title = "{The Propagation of Uncertainties in Stellar Population Synthesis Modeling. III. Model Calibration, Comparison, and Evaluation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0911.3151},
 keywords = {galaxies: evolution, galaxies: stellar content, stars: evolution},
     year = 2010,
    month = apr,
   volume = 712,
    pages = {833-857},
      doi = {10.1088/0004-637X/712/2/833},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...712..833C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{foreman_mackey2014,
  author       = {Dan Foreman-Mackey and
                  Jonathan Sick and
                  Ben Johnson},
  title        = {python-fsps: Python bindings to FSPS (v0.1.1)},
  month        = oct,
  year         = 2014,
  doi          = {10.5281/zenodo.12157},
  url          = {https://doi.org/10.5281/zenodo.12157}
}

@ARTICLE{barrera2018,
       author = {{Barrera-Ballesteros}, J.~K. and {Heckman}, T. and {S{\'a}nchez}, S.~F. and
         {Zakamska}, N.~L. and {Cleary}, J. and {Zhu}, G. and {Brinkmann}, J. and
         {Drory}, N. and {THE MaNGA TEAM}},
        title = "{SDSS-IV MaNGA: What Shapes the Distribution of Metals in Galaxies? Exploring the Roles of the Local Gas Fraction and Escape Velocity}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: statistics, surveys, techniques: imaging spectroscopy, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Jan",
       volume = {852},
       number = {2},
          eid = {74},
        pages = {74},
          doi = {10.3847/1538-4357/aa9b31},
archivePrefix = {arXiv},
       eprint = {1711.10492},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...852...74B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{barrera2015,
       author = {{Barrera-Ballesteros}, J.~K. and {Garc{\'\i}a-Lorenzo}, B. and
         {Falc{\'o}n-Barroso}, J. and {van de Ven}, G. and {Lyubenova}, M. and
         {Wild}, V. and {M{\'e}ndez-Abreu}, J. and {S{\'a}nchez}, S.~F. and
         {Marquez}, I. and {Masegosa}, J. and {Monreal-Ibero}, A. and
         {Ziegler}, B. and {del Olmo}, A. and {Verdes-Montenegro}, L. and
         {Garc{\'\i}a-Benito}, R. and {Husemann}, B. and {Mast}, D. and
         {Kehrig}, C. and {Iglesias-Paramo}, J. and {Marino}, R.~A. and
         {Aguerri}, J.~A.~L. and {Walcher}, C.~J. and {V{\'\i}lchez}, J.~M. and
         {Bomans}, D.~J. and {Cortijo-Ferrero}, C. and
         {Gonz{\'a}lez Delgado}, R.~M. and {Bland-Hawthorn}, J. and
         {McIntosh}, D.~H. and {Bekerait{\.{e}}}, S.},
        title = "{Tracing kinematic (mis)alignments in CALIFA merging galaxies. Stellar and ionized gas kinematic orientations at every merger stage}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: interactions, galaxies: kinematics and dynamics, galaxies: statistics, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Oct",
       volume = {582},
          eid = {A21},
        pages = {A21},
          doi = {10.1051/0004-6361/201424935},
archivePrefix = {arXiv},
       eprint = {1506.03819},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..21B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{codis2015,
       author = {{Codis}, Sandrine and {Pichon}, Christophe and {Pogosyan}, Dmitry},
        title = "{Spin alignments within the cosmic web: a theory of constrained tidal torques near filaments}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, cosmology: theory, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "Oct",
       volume = {452},
       number = {4},
        pages = {3369-3393},
          doi = {10.1093/mnras/stv1570},
archivePrefix = {arXiv},
       eprint = {1504.06073},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.452.3369C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pichon2011,
       author = {{Pichon}, C. and {Pogosyan}, D. and {Kimm}, T. and {Slyz}, A. and
         {Devriendt}, J. and {Dubois}, Y.},
        title = "{Rigging dark haloes: why is hierarchical galaxy formation consistent with the inside-out build-up of thin discs?}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: statistics, galaxies: structure, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2011",
        month = "Dec",
       volume = {418},
       number = {4},
        pages = {2493-2507},
          doi = {10.1111/j.1365-2966.2011.19640.x},
archivePrefix = {arXiv},
       eprint = {1105.0210},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.418.2493P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laigle2015,
       author = {{Laigle}, C. and {Pichon}, C. and {Codis}, S. and {Dubois}, Y. and
         {Le Borgne}, D. and {Pogosyan}, D. and {Devriendt}, J. and
         {Peirani}, S. and {Prunet}, S. and {Rouberol}, S. and {Slyz}, A. and
         {Sousbie}, T.},
        title = "{Swirling around filaments: are large-scale structure vortices spinning up dark haloes?}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: formation, galaxies: haloes, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "Jan",
       volume = {446},
       number = {3},
        pages = {2744-2759},
          doi = {10.1093/mnras/stu2289},
archivePrefix = {arXiv},
       eprint = {1310.3801},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.2744L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blanton2011,
   author = {{Blanton}, M.~R. and {Kazin}, E. and {Muna}, D. and {Weaver}, B.~A. and 
	{Price-Whelan}, A.},
    title = "{Improved Background Subtraction for the Sloan Digital Sky Survey Images}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1105.1960},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, galaxies: photometry, methods: data analysis, techniques: image processing},
     year = 2011,
    month = jul,
   volume = 142,
      eid = {31},
    pages = {31},
      doi = {10.1088/0004-6256/142/1/31},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142...31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nelson2019,
       author = {{Nelson}, Dylan and {Springel}, Volker and {Pillepich}, Annalisa and
         {Rodriguez-Gomez}, Vicente and {Torrey}, Paul and {Genel}, Shy and
         {Vogelsberger}, Mark and {Pakmor}, Ruediger and {Marinacci}, Federico and
         {Weinberger}, Rainer and {Kelley}, Luke and {Lovell}, Mark and
         {Diemer}, Benedikt and {Hernquist}, Lars},
        title = "{The IllustrisTNG simulations: public data release}",
      journal = {Computational Astrophysics and Cosmology},
     keywords = {Methods: data analysis, Methods: numerical, Galaxies: formation, Galaxies: evolution, Data management systems, Data access methods, Distributed architectures, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2019",
        month = "May",
       volume = {6},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.1186/s40668-019-0028-x},
archivePrefix = {arXiv},
       eprint = {1812.05609},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ComAC...6....2N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
